Clean Label Attacks against SLU Systems

Poisoning backdoor attacks involve an adversary manipulating the training data to induce certain behaviors in the victim model by inserting a trigger in the signal at inference time. We adapted clean label backdoor (CLBD)-data poisoning attacks, which do not modify the training labels, on state-of-the-art speech recognition models that support/perform a Spoken Language Understanding task, achieving 99.8% attack success rate by poisoning 10% of the training data. We analyzed how varying the signal-strength of the poison, percent of samples poisoned, and choice of trigger impact the attack. We also found that CLBD attacks are most successful when applied to training samples that are inherently hard for a proxy model. Using this strategy, we achieved an attack success rate of 99.3% by poisoning a meager 1.5% of the training data. Finally, we applied two previously developed defenses against gradient-based attacks, and found that they attain mixed success against poisoning.

==> my_bib.backup.tex <==
%%% Poisoning Attacks
@inproceedings{Big,
author = {Biggio, Battista and Nelson, Blaine and Laskov, Pavel},
title = {Poisoning attacks against support vector machines},
year = {2012},
isbn = {9781450312851},
publisher = {Omnipress},
address = {Madison, WI, USA},
abstract = {We investigate a family of poisoning attacks against Support Vector Machines (SVM). Such attacks inject specially crafted training data that increases the SVM's test error. Central to the motivation for these attacks is the fact that most learning algorithms assume that their training data comes from a natural or well-behaved distribution. However, this assumption does not generally hold in security-sensitive settings. As we demonstrate, an intelligent adversary can, to some extent, predict the change of the SVM's decision function due to malicious input and use this ability to construct malicious data.The proposed attack uses a gradient ascent strategy in which the gradient is computed based on properties of the SVM's optimal solution. This method can be kernelized and enables the attack to be constructed in the input space even for non-linear kernels. We experimentally demonstrate that our gradient ascent procedure reliably identifies good local maxima of the non-convex validation error surface, which significantly increases the classifier's test error.},
booktitle = {Proceedings of the 29th International Coference on International Conference on Machine Learning},
pages = {1467–1474},
numpages = {8},
location = {Edinburgh, Scotland},
series = {ICML'12}
}

@article{li2024multi,
  title={Multi-Trigger Backdoor Attacks: More Triggers, More Threats},
  author={Li, Yige and Ma, Xingjun and He, Jiabo and Huang, Hanxun and Jiang, Yu-Gang},
  journal={arXiv preprint arXiv:2401.15295},
  year={2024}
}


@inproceedings{thebaud2023clustering,
  title={Clustering Unsupervised Representations as Defense Against Poisoning Attacks on Speech Commands Classification System},
  author={Thebaud, Thomas and Joshi, Sonal and Li, Henry and Sustek, Martin and Villalba, Jes{\'u}s and Khudanpur, Sanjeev and Dehak, Najim},
  booktitle={2023 IEEE Automatic Speech Recognition and Understanding Workshop (ASRU)},
  pages={1--8},
  year={2023},
  organization={IEEE}
}


@article{Badnets,
  title={BadNets: Evaluating Backdooring Attacks on Deep Neural Networks},
  author={Tianyu Gu and Kang Liu and Brendan Dolan-Gavitt and Siddharth Garg},
  journal={IEEE Access},
  year={2019},
  volume={7},
  pages={47230-47244}
}

@article{CV, title={Poisoning-Based Backdoor Attacks in Computer Vision}, volume={37}, url={https://ojs.aaai.org/index.php/AAAI/article/view/26921}, DOI={10.1609/aaai.v37i13.26921}, abstractNote={Recent studies demonstrated that the training process of deep neural networks (DNNs) is vulnerable to backdoor attacks if third-party training resources (e.g., samples) are adopted. Specifically, the adversaries intend to embed hidden backdoors into DNNs, where the backdoor can be activated by pre-defined trigger patterns and leading malicious model predictions. My dissertation focuses on poisoning-based backdoor attacks in computer vision. Firstly, I study and propose more stealthy and effective attacks against image classification tasks in both physical and digital spaces. Secondly, I reveal the backdoor threats in visual object tracking, which is representative of critical video-related tasks. Thirdly, I explore how to exploit backdoor attacks as watermark techniques for positive purposes. I design a Python toolbox (i.e., BackdoorBox) that implements representative and advanced backdoor attacks and defenses under a unified and flexible framework, based on which to provide a comprehensive benchmark of existing methods at the end.}, number={13}, journal={Proceedings of the AAAI Conference on Artificial Intelligence}, author={Li, Yiming}, year={2023}, month={Sep.}, pages={16121-16122} }

@inproceedings{
Badtrack,
title={BadTrack: A Poison-Only Backdoor Attack on Visual Object Tracking},
author={Bin Huang and Jiaqian Yu and Yiwei Chen and Siyang Pan and Qiang Wang and Zhi Wang},
booktitle={Thirty-seventh Conference on Neural Information Processing Systems},
year={2023},
url={https://openreview.net/forum?id=W9pJx9sFCh}
}

@inproceedings{
LLM,
title={Forcing Generative Models to Degenerate Ones: The Power of Data Poisoning Attacks},
author={Shuli Jiang and Swanand Kadhe and Yi Zhou and Ling Cai and Nathalie Baracaldo},
booktitle={NeurIPS 2023 Workshop on Backdoors in Deep Learning - The Good, the Bad, and the Ugly},
year={2023},
url={https://openreview.net/forum?id=8R4z3XZt5J}
}

@ARTICLE{audio,
  author={Ge, Yunjie and Wang, Qian and Yu, Jiayuan and Shen, Chao and Li, Qi},
  journal={IEEE Communications Magazine}, 
  title={Data Poisoning and Backdoor Attacks on Audio Intelligence Systems}, 
  year={2023},
  volume={61},
  number={12},
  pages={176-182},
  keywords={Training;Data models;Speech recognition;Feature extraction;Behavioral sciences;Training data;Computational modeling},
  doi={10.1109/MCOM.012.2200596}}

%%% Much data needed
@misc{whisper-style,
      title={Reproducing Whisper-Style Training Using an Open-Source Toolkit and Publicly Available Data}, 
      author={Yifan Peng and Jinchuan Tian and Brian Yan and Dan Berrebbi and Xuankai Chang and Xinjian Li and Jiatong Shi and Siddhant Arora and William Chen and Roshan Sharma and Wangyou Zhang and Yui Sudo and Muhammad Shakeel and Jee-weon Jung and Soumi Maiti and Shinji Watanabe},
      year={2023},
      eprint={2309.13876},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}%ASR models use data crawled from the internet

@misc{gpt-3,
      title={Language Models are Few-Shot Learners}, 
      author={Tom B. Brown and Benjamin Mann and Nick Ryder and Melanie Subbiah and Jared Kaplan and Prafulla Dhariwal and Arvind Neelakantan and Pranav Shyam and Girish Sastry and Amanda Askell and Sandhini Agarwal and Ariel Herbert-Voss and Gretchen Krueger and Tom Henighan and Rewon Child and Aditya Ramesh and Daniel M. Ziegler and Jeffrey Wu and Clemens Winter and Christopher Hesse and Mark Chen and Eric Sigler and Mateusz Litwin and Scott Gray and Benjamin Chess and Jack Clark and Christopher Berner and Sam McCandlish and Alec Radford and Ilya Sutskever and Dario Amodei},
      year={2020},
      eprint={2005.14165},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}%LMs use data crawled from the internet

@INPROCEEDINGS {practical,
author = {N. Carlini and M. Jagielski and C. Choquette-Choo and D. Paleka and W. Pearce and H. Anderson and A. Terzis and K. Thomas and F. Tramèr},
booktitle = {2024 IEEE Symposium on Security and Privacy (SP)},
title = {Poisoning Web-Scale Training Datasets is Practical},
year = {2024},
volume = {},
issn = {2375-1207},
pages = {176-176},
abstract = {Deep learning models are often trained on distributed, web-scale datasets crawled from the internet. In this paper, we introduce two new dataset poisoning attacks that intentionally introduce malicious examples to a model’s performance. Our attacks are immediately practical and could, today, poison 10 popular datasets. Our first attack, split-view poisoning, exploits the mutable nature of internet content to ensure a dataset annotator’s initial view of the dataset differs from the view downloaded by subsequent clients. By exploiting specific invalid trust assumptions, we show how we could have poisoned 0.01% of the LAION-400M or COYO-700M datasets for just $60 USD. Our second attack, frontrunning poisoning, targets web-scale datasets that periodically snapshot crowdsourced content—such as Wikipedia—where an attacker only needs a time-limited window to inject malicious examples. In light of both attacks, we notify the maintainers of each affected dataset and recommended several low-overhead defenses.},
keywords = {},
doi = {10.1109/SP54263.2024.00094},
url = {https://doi.ieeecomputersociety.org/10.1109/SP54263.2024.00094},
publisher = {IEEE Computer Society},
address = {Los Alamitos, CA, USA},
month = {may}
}%Poisoning attacks are realistic

%%% Clean label attacks work

@misc{clean-label,
      title={Label-Consistent Backdoor Attacks}, 
      author={Alexander Turner and Dimitris Tsipras and Aleksander Madry},
      year={2019},
      eprint={1912.02771},
      archivePrefix={arXiv},
      primaryClass={stat.ML}
}

@inproceedings{poison-frogs,
 author = {Shafahi, Ali and Huang, W. Ronny and Najibi, Mahyar and Suciu, Octavian and Studer, Christoph and Dumitras, Tudor and Goldstein, Tom},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {S. Bengio and H. Wallach and H. Larochelle and K. Grauman and N. Cesa-Bianchi and R. Garnett},
 pages = {},
 publisher = {Curran Associates, Inc.},
 title = {Poison Frogs! Targeted Clean-Label Poisoning Attacks on Neural Networks},
 url = {https://proceedings.neurips.cc/paper_files/paper/2018/file/22722a343513ed45f14905eb07621686-Paper.pdf},
 volume = {31},
 year = {2018}
}


%%% Poisoning attacks
@article{biggio2012poisoning,
  title={Poisoning attacks against support vector machines},
  author={Biggio, Battista and Nelson, Blaine and Laskov, Pavel},
  journal={arXiv preprint arXiv:1206.6389},
  year={2012}
}%not on DNN, but on SVM (but classic as it seems)

@inproceedings{trojaning,
  added-at = {2023-12-13T06:56:08.000+0100},
  author = {Liu, Yingqi and Ma, Shiqing and Aafer, Yousra and Lee, Wen-Chuan and Zhai, Juan and Wang, Weihang and Zhang, Xiangyu},
  biburl = {https://www.bibsonomy.org/bibtex/2de62625641e16e2e842b9d03861075b4/admin},
  booktitle = {NDSS},
  ee = {http://wp.internetsociety.org/ndss/wp-content/uploads/sites/25/2018/02/ndss2018_03A-5_Liu_paper.pdf},
  interhash = {b369462c9abaa51874afd3205deb2f82},
  intrahash = {de62625641e16e2e842b9d03861075b4},
  keywords = {},
  publisher = {The Internet Society},
  timestamp = {2023-12-13T06:56:08.000+0100},
  title = {Trojaning Attack on Neural Networks.},
  url = {http://dblp.uni-trier.de/db/conf/ndss/ndss2018.html#LiuMALZW018},
  year = 2018
}%poisoning attack (generic)

@INPROCEEDINGS{trojanmodel,
  author={Zong, Wei and Chow, Yang-Wai and Susilo, Willy and Do, Kien and Venkatesh, Svetha},
  booktitle={2023 IEEE Symposium on Security and Privacy (SP)}, 
  title={TrojanModel: A Practical Trojan Attack against Automatic Speech Recognition Systems}, 
  year={2023},
  volume={},
  number={},
  pages={1667-1683},
  keywords={Deep learning;Privacy;Acoustics;Trojan horses;Security;Automatic speech recognition;Microphones;adversarial machine learning;automatic speech recognition;backdoor;deep learning;Trojan},
  doi={10.1109/SP46215.2023.10179331}
}%dirty label agasint ASR

@article{venowave,
  title={VENOMAVE: Clean-label poisoning against speech recognition},
  author={Aghakhani, Hojjat and Eisenhofer, Thorsten and Sch{\"o}nherr, Lea and Kolossa, Dorothea and Holz, Thorsten and Kruegel, Christopher and Vigna, Giovanni},
  journal={Computing Research Repository (CoRR), abs/2010.10682},
  year={2020}
}%attack on speech commands


@article{yang2017generative,
  title={Generative poisoning attack method against neural networks},
  author={Yang, Chaofei and Wu, Qing and Li, Hai and Chen, Yiran},
  journal={arXiv preprint arXiv:1703.01340},
  year={2017}
}% against MNIST

@inproceedings{zhai2021backdoor,
  title={Backdoor attack against speaker verification},
  author={Zhai, Tongqing and Li, Yiming and Zhang, Ziqi and Wu, Baoyuan and Jiang, Yong and Xia, Shu-Tao},
  booktitle={ICASSP 2021-2021 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={2560--2564},
  year={2021},
  organization={IEEE}
}%Speaker verification


@inproceedings{blackbox-nmt,
author = {Xu, Chang and Wang, Jun and Tang, Yuqing and Guzm\'{a}n, Francisco and Rubinstein, Benjamin I. P. and Cohn, Trevor},
title = {A Targeted Attack on Black-Box Neural Machine Translation with Parallel Data Poisoning},
year = {2021},
isbn = {9781450383127},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3442381.3450034},
doi = {10.1145/3442381.3450034},
abstract = {As modern neural machine translation (NMT) systems have been widely deployed, their security vulnerabilities require close scrutiny. Most recently, NMT systems have been found vulnerable to targeted attacks which cause them to produce specific, unsolicited, and even harmful translations. These attacks are usually exploited in a white-box setting, where adversarial inputs causing targeted translations are discovered for a known target system. However, this approach is less viable when the target system is black-box and unknown to the adversary (e.g., secured commercial systems). In this paper, we show that targeted attacks on black-box NMT systems are feasible, based on poisoning a small fraction of their parallel training data. We show that this attack can be realised practically via targeted corruption of web documents crawled to form the system’s training data. We then analyse the effectiveness of the targeted poisoning in two common NMT training scenarios: the from-scratch training and the pre-train \& fine-tune paradigm. Our results are alarming: even on the state-of-the-art systems trained with massive parallel data (tens of millions), the attacks are still successful (over 50\% success rate) under surprisingly low poisoning budgets (e.g., 0.006\%). Lastly, we discuss potential defences to counter such attacks.},
booktitle = {Proceedings of the Web Conference 2021},
pages = {3638–3650},
numpages = {13},
keywords = {neural machine translation, data poisoning, black-box attacks},
location = {Ljubljana, Slovenia},
series = {WWW '21}
}%against black box nmt

@inproceedings{nmt,
    title = "Putting words into the system{'}s mouth: A targeted attack on neural machine translation using monolingual data poisoning",
    author = "Wang, Jun  and
      Xu, Chang  and
      Guzm{\'a}n, Francisco  and
      El-Kishky, Ahmed  and
      Tang, Yuqing  and
      Rubinstein, Benjamin  and
      Cohn, Trevor",
    editor = "Zong, Chengqing  and
      Xia, Fei  and
      Li, Wenjie  and
      Navigli, Roberto",
    booktitle = "Findings of the Association for Computational Linguistics: ACL-IJCNLP 2021",
    month = aug,
    year = "2021",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2021.findings-acl.127",
    doi = "10.18653/v1/2021.findings-acl.127",
    pages = "1463--1473",
}%against nmt


@misc{backdoor,
      title={Backdoor Learning: A Survey}, 
      author={Yiming Li and Yong Jiang and Zhifeng Li and Shu-Tao Xia},
      year={2022},
      eprint={2007.08745},
      archivePrefix={arXiv},
      primaryClass={cs.CR}
}%survey

%% Victim Model
@misc{pruned,
      title={Pruned RNN-T for fast, memory-efficient ASR training}, 
      author={Fangjun Kuang and Liyong Guo and Wei Kang and Long Lin and Mingshuang Luo and Zengwei Yao and Daniel Povey},
      year={2022},
      eprint={2206.13236},
      archivePrefix={arXiv},
      primaryClass={eess.AS}
}%Pruned RNN-T

@inproceedings{fluent,
  author    = {Loren Lugosch and
               Mirco Ravanelli and
               Patrick Ignoto and
               Vikrant Singh Tomar and
               Yoshua Bengio},
  editor    = {Gernot Kubin and
               Zdravko Kacic},
  title     = {Speech Model Pre-Training for End-to-End Spoken Language Understanding},
  booktitle = {Proc. of Interspeech},
  pages     = {814--818},
  year      = {2019},
}%Fluent Speech Commands dataset

@article{dirty,
  title={Targeted backdoor attacks on deep learning systems using data poisoning},
  author={Chen, Xinyun and Liu, Chang and Li, Bo and Lu, Kimberly and Song, Dawn},
  journal={arXiv preprint arXiv:1712.05526},
  year={2017}
}%Targeted backdoor on deeplearning

@misc{rnn-t,
      title={Sequence Transduction with Recurrent Neural Networks}, 
      author={Alex Graves},
      year={2012},
      eprint={1211.3711},
      archivePrefix={arXiv},
      primaryClass={cs.NE}
}%RNN-T Model

@misc{conformer,
      title={Conformer: Convolution-augmented Transformer for Speech Recognition}, 
      author={Anmol Gulati and James Qin and Chung-Cheng Chiu and Niki Parmar and Yu Zhang and Jiahui Yu and Wei Han and Shibo Wang and Zhengdong Zhang and Yonghui Wu and Ruoming Pang},
      year={2020},
      eprint={2005.08100},
      archivePrefix={arXiv},
      primaryClass={eess.AS}
}%Conformer Model


%% Ranked attack
@misc{ranked,
      title={Confidence-driven Sampling for Backdoor Attacks}, 
      author={Pengfei He and Han Xu and Yue Xing and Jie Ren and Yingqian Cui and Shenglai Zeng and Jiliang Tang and Makoto Yamada and Mohammad Sabokrou},
      year={2023},
      eprint={2310.05263},
      archivePrefix={arXiv},
      primaryClass={cs.CR}
}


%% Transferability of adversarial samples
@misc{transferability,
      title={Closer Look at the Transferability of Adversarial Examples: How They Fool Different Models Differently}, 
      author={Futa Waseda and Sosuke Nishikawa and Trung-Nghia Le and Huy H. Nguyen and Isao Echizen},
      year={2022},
      eprint={2112.14337},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@INPROCEEDINGS{improve_transferability,
  author={Xu, Yinhu and Chu, Qi and Yu, Nenghai},
  booktitle={2021 IEEE Sixth International Conference on Data Science in Cyberspace (DSC)}, 
  title={Improving the Transferability of Adversarial Examples with Advanced Diversity-Ensemble Method}, 
  year={2021},
  volume={},
  number={},
  pages={219-225},
  keywords={Conferences;Cyberspace;Data science;Benchmark testing;Market research;Robustness;adversarial examples;black-box attack;transferability;input diversity},
  doi={10.1109/DSC53577.2021.00037}}

@inproceedings{alexa,
 author = {Li, Juncheng and Qu, Shuhui and Li, Xinjian and Szurley, Joseph and Kolter, J. Zico and Metze, Florian},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {H. Wallach and H. Larochelle and A. Beygelzimer and F. d\textquotesingle Alch\'{e}-Buc and E. Fox and R. Garnett},
 pages = {},
 publisher = {Curran Associates, Inc.},
 title = {Adversarial Music: Real world Audio Adversary against Wake-word Detection System},
 url = {https://proceedings.neurips.cc/paper_files/paper/2019/file/ebbdfea212e3a756a1fded7b35578525-Paper.pdf},
 volume = {32},
 year = {2019}
}

@article{joshi2022defense,
  title={Defense against adversarial attacks on hybrid speech recognition using joint adversarial fine-tuning with denoiser},
  author={Joshi, Sonal and Kataria, Saurabh and Shao, Yiwen and Zelasko, Piotr and Villalba, Jes{\'u}s and Khudanpur, Sanjeev and Dehak, Najim},
  journal={Interspeech},
  year={2022}
}

@article{chung2018voxceleb2,
  title={Voxceleb2: Deep speaker recognition},
  author={Chung, Joon Son and Nagrani, Arsha and Zisserman, Andrew},
  journal={arXiv preprint arXiv:1806.05622},
  year={2018}
}

@inproceedings{panayotov2015librispeech,
  title={Librispeech: an {ASR} corpus based on public domain audio books},
  author={Panayotov, Vassil and Chen, Guoguo and Povey, Daniel and Khudanpur, Sanjeev},
  booktitle={2015 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={5206--5210},
  year={2015},
  organization={IEEE}
}

@misc{joshi2024unraveling,
      title={Unraveling Adversarial Examples against Speaker Identification -- Techniques for Attack Detection and Victim Model Classification}, 
      author={Sonal Joshi and Thomas Thebaud and Jesús Villalba and Najim Dehak},
      year={2024},
      eprint={2402.19355},
      archivePrefix={arXiv},
      primaryClass={cs.SD}
}


@misc{random,
      title={Mitigating Adversarial Effects Through Randomization}, 
      author={Cihang Xie and Jianyu Wang and Zhishuai Zhang and Zhou Ren and Alan Yuille},
      year={2018},
      eprint={1711.01991},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}


@INPROCEEDINGS{hard_for_human,
  author={Baracaldo, Nathalie and Ahmed, Farhan and Eykholt, Kevin and Zhou, Yi and Priya, Shriti and Lee, Taesung and Kadhe, Swanand and Tan, Mike and Polavaram, Sridevi and Suggs, Sterling and Gao, Yuyang and Slater, David},
  booktitle={2023 IEEE Security and Privacy Workshops (SPW)}, 
  title={Benchmarking the Effect of Poisoning Defenses on the Security and Bias of Deep Learning Models}, 
  year={2023},
  volume={},
  number={},
  pages={45-56},
  keywords={Measurement;Training;Toxicology;Machine learning algorithms;Training data;Data models;Robustness;AI-secuirty;AI-poisoning;AI-defenses;AI-trustworthiness},
  doi={10.1109/SPW59333.2023.00010}}

@inproceedings{peri2020deep,
  title={Deep k-nn defense against clean-label data poisoning attacks},
  author={Peri, Neehar and Gupta, Neal and Huang, W Ronny and Fowl, Liam and Zhu, Chen and Feizi, Soheil and Goldstein, Tom and Dickerson, John P},
  booktitle={Computer Vision--ECCV 2020 Workshops: Glasgow, UK, August 23--28, 2020, Proceedings, Part I 16},
  pages={55--70},
  year={2020},
  organization={Springer}
}

@article{geiping2021doesn,
  title={What doesn't kill you makes you robust (er): How to adversarially train against data poisoning},
  author={Geiping, Jonas and Fowl, Liam and Somepalli, Gowthami and Goldblum, Micah and Moeller, Michael and Goldstein, Tom},
  journal={arXiv preprint arXiv:2102.13624},
  year={2021}
}

@inproceedings{hammoudeh2021simple,
  title={Simple, Attack-Agnostic Defense Against Targeted Training Set Attacks Using Cosine Similarity},
  author={Hammoudeh, Zayd and Lowd, Daniel},
  journal={ICML Workshop on Uncertainty in Deep Learning (UDL)},
  year={2021}
}


@InProceedings{pmlr-v162-yang22j,
  title = 	 {Not All Poisons are Created Equal: Robust Training against Data Poisoning},
  author =       {Yang, Yu and Liu, Tian Yu and Mirzasoleiman, Baharan},
  booktitle = 	 {Proceedings of the 39th International Conference on Machine Learning},
  pages = 	 {25154--25165},
  year = 	 {2022},
  editor = 	 {Chaudhuri, Kamalika and Jegelka, Stefanie and Song, Le and Szepesvari, Csaba and Niu, Gang and Sabato, Sivan},
  volume = 	 {162},
  series = 	 {Proceedings of Machine Learning Research},
  month = 	 {17--23 Jul},
  publisher =    {PMLR},
  pdf = 	 {https://proceedings.mlr.press/v162/yang22j/yang22j.pdf},
  url = 	 {https://proceedings.mlr.press/v162/yang22j.html},
  abstract = 	 {Data poisoning causes misclassification of test time target examples, by injecting maliciously crafted samples in the training data. Existing defenses are often effective only against a specific type of targeted attack, significantly degrade the generalization performance, or are prohibitive for standard deep learning pipelines. In this work, we propose an efficient defense mechanism that significantly reduces the success rate of various data poisoning attacks, and provides theoretical guarantees for the performance of the model. Targeted attacks work by adding bounded perturbations to a randomly selected subset of training data to match the targets’ gradient or representation. We show that: (i) under bounded perturbations, only a number of poisons can be optimized to have a gradient that is close enough to that of the target and make the attack successful; (ii) such effective poisons move away from their original class and get isolated in the gradient space; (iii) dropping examples in low-density gradient regions during training can successfully eliminate the effective poisons, and guarantees similar training dynamics to that of training on full data. Our extensive experiments show that our method significantly decreases the success rate of state-of-the-art targeted attacks, including Gradient Matching and Bullseye Polytope, and easily scales to large datasets.}
}

